Bringing data minimization to digital wallets at scale with general-purpose zero-knowledge proofs

Today, digital identity management for individuals is either inconvenient and error-prone or creates undesirable lock-in effects and violates privacy and security expectations. These shortcomings inhibit the digital transformation in general and seem particularly concerning in the context of novel applications such as access control for decentralized autonomous organizations and identification in the Metaverse. Decentralized or self-sovereign identity (SSI) aims to offer a solution to this dilemma by empowering individuals to manage their digital identity through machine-verifiable attestations stored in a "digital wallet" application on their edge devices. However, when presented to a relying party, these attestations typically reveal more attributes than required and allow tracking end users' activities. Several academic works and practical solutions exist to reduce or avoid such excessive information disclosure, from simple selective disclosure to data-minimizing anonymous credentials based on zero-knowledge proofs (ZKPs). We first demonstrate that the SSI solutions that are currently built with anonymous credentials still lack essential features such as scalable revocation, certificate chaining, and integration with secure elements. We then argue that general-purpose ZKPs in the form of zk-SNARKs can appropriately address these pressing challenges. We describe our implementation and conduct performance tests on different edge devices to illustrate that the performance of zk-SNARK-based anonymous credentials is already practical. We also discuss further advantages that general-purpose ZKPs can easily provide for digital wallets, for instance, to create "designated verifier presentations" that facilitate new design options for digital identity infrastructures that previously were not accessible because of the threat of man-in-the-middle attacks.

==> Tables/SplitTable.tex <==

\renewcommand{\arraystretch}{1.2}
\begin{table*}[!htb]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{r|r||r|r|r|r|r|r|r|r}
        \multicolumn{2}{c||}{\textbf{Building blocks}} & \multicolumn{8}{c}{\textbf{Number of occurrences in corresponding scenario and contribution to number of constraints}} \\\hline\hline
        \textbf{Component} & \textbf{\# constraints} & \multicolumn{2}{c|}{\textbf{I}} & \multicolumn{2}{c|}{\textbf{II}} & \multicolumn{2}{c|}{\textbf{III}} & \multicolumn{2}{c}{\textbf{IV}} \\\hline
        & & \# Occurrences & Constr. & \# Occ. & Constr. & \# Occ. & Constr. & \# Occurrences & Constr. \\\hline\hline
        Selector & 5 & 4 + 13 = 17 & 85 & 17 & 85 & 22 & 110 & 4 + 3 * 13 = 43 & 215 \\\hline
        %Num2Bits(3) & 3 & 1 & 3 & 1 & 3 & 1 & 3 & 3 & 9 & 1 & 3 & 3 & 9 \\ \hline
        Range proof & 252 & 1 & 252 & 1 & 252 & 1 & 252 & 3 & 756 \\\hline
        Division with rest & 252 & 1 & 252 & 1 & 252 & 1 & 252 & 3 & 756 \\\hline
        Poseidon hash & 240 & 1 + 4 + 7 + 13 = 25 & 6,000 & 28 & 6,720 & 30 & 7,200 & 4 + 3 * (1 + 7 + 13) + 2 * 2 = 71 & 17,040 \\\hline
        extractKthBit & 1,012 & 1 & 1,012 & 1 & 1,012 & 1 & 1,012 & 3 & 3,036  \\\hline
        \ac{eddsa} signature & 4,218 & 1 + 1 = 2 & 8,436 & 2 & 8,436 & 2 & 8,436 & 1 + 3 * 1 = 4 & 16,872 \\\hline
        \ac{sha256} hash & 29,636 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\\hline
        \ac{ecdsa} signature & 163,239$^\ast$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        & (1,508,136) & & & & & & & \\\hline\hline
        \multicolumn{2}{r||}{\textbf{Total number of constraints}} & \multicolumn{2}{r|}{\textbf{16,037}} & \multicolumn{2}{r|}{\textbf{16,757}} & \multicolumn{2}{r|}{\textbf{17,262}} & \multicolumn{2}{r}{\textbf{38,915}}
        \end{tabular}
    } \\[0.5cm]
    \raggedright
    \resizebox{0.675\linewidth}{!}{%
    \begin{tabular}{r|r||r|r|r|r|r|r}
        \multicolumn{2}{c||}{\textbf{Building blocks}} & \multicolumn{6}{c}{\textbf{\# Occ. in scenario and contr. to \# Constr.}} \\\hline\hline
        \textbf{Component} & \textbf{\# constraints} & \multicolumn{2}{c|}{\textbf{V}} & \multicolumn{2}{c|}{\textbf{VI}} & \multicolumn{2}{c}{\textbf{VII}} \\\hline
        & & \# Occ. & Constr. & \# Occ. & Constr. & \# Occ. & Constr. \\\hline\hline
        Selector & 5 & 17 & 85 & 17 & 85 & 43 & 215 \\\hline
        Range proof & 252 & 1 & 252 & 1 & 252 & 3 & 756 \\\hline
        Division with rest & 252 & 1 & 252 & 1 & 252 & 3 & 756 \\\hline
        Poseidon hash & 240 & 25 & 6000 & 0 & 0 & 0 & 0 \\\hline
        extractKthBit & 1,012 & 1 & 1,012 & 1 & 1,012 & 3 & 3,036 \\\hline
        \ac{eddsa} signature & 4,218 & 1 + 3 * 1 = 4 & 16,872 & 1 & 4,218 & 0 & 0\\\hline
        \ac{sha256} hash & 29,636 & 0 & 0 & 25 & 740,900 & 71 & 2,104,156 \\\hline
        \ac{ecdsa} signature & 163,239$^\ast$ & 1 & 163,239 & 2 & 326,478 & 4 & 652,956 \\
        & (1,508,136) & & & & & & \\\hline\hline
        \multicolumn{2}{r||}{\textbf{Total number of constraints}} &  \multicolumn{2}{r|}{\textbf{175,058}} & \multicolumn{2}{r|}{\textbf{1,068,979}} & \multicolumn{2}{r}{\textbf{2,761,875}}
        \end{tabular}
    }
   \caption{Number of constraints for the most relevant basic building blocks and their occurrence in the basic scenarios. For instance, a non-revocation proof with the Poseidon hash in a revocation registry representing 2~million credentials involves 13~Poseidon hashes and Selectors, an integer division with rest, and an extractKthBit component. We ignore the constraints associated with small operations, such as converting an attribute position into a Merkle path via the Num2Bits component, which adds only $1$ constraint per hash in a Merkle proof. 
   Note that combining several components in one circuit can even decrease the total number of non-linear constraints that are a proxy for proving complexity and in particular proving time~\citep{albert2022distilling}, although no significant reduction can be observed. \\ ~\\\scriptsize{$^\ast$ With preprocessing inputs.}}
    \label{tab:componentsAndCosts}
\end{table*}
